Continuously Indexed Domain Adaptation

Existing domain adaptation focuses on transferring knowledge between domains with categorical indices (e.g., between datasets A and B). However, many tasks involve continuously indexed domains. For example, in medical applications, one often needs to transfer disease analysis and prediction across patients of different ages, where age acts as a continuous domain index. Such tasks are challenging for prior domain adaptation methods since they ignore the underlying relation among domains. In this paper, we propose the first method for continuously indexed domain adaptation. Our approach combines traditional adversarial adaptation with a novel discriminator that models the encoding-conditioned domain index distribution. Our theoretical analysis demonstrates the value of leveraging the domain index to generate invariant features across a continuous range of domains. Our empirical results show that our approach outperforms the state-of-the-art domain adaption methods on both synthetic and real-world medical datasets.

==> source/sup_matching.tex <==
\section{Matching $p(u | \z)$ versus Matching $p(\z | u)$} 
In general, matching the entire $p(u | \z)$ for any $\z$ is equivalent to matching the entire $p(\z | u)$ for any $u$. This is because $p(u | \z) = p(u) \iff p(\z | u) = p(\z) \iff u \indep \z$. However, matching the mean and variance of $p(u | \z)$ for any $\z$ is \textbf{different} from matching the mean and variance of $p(\z | u)$ for any $u$. Considering the dimension of $\z$ is much higher than that of $u$, the former is actually \textbf{stronger} alignment. 



To see this, consider a simplified case where $\z \in \{1,2,3,4\}^{100}$ and $u \in  \{1,2,3,4\}$. Matching the mean and variance of $p(u | \z)$ requires matching the mean and variance of $4^{100}$ univariate distributions, i.e., $2\times 4^{100}$ parameters in total. On the other hand, Matching the mean and variance of $p(\z | u)$ only requires matching the mean and variance of $4$ $100$-dimensional distributions, i.e., $400$ parameters in total. Therefore the former implies stronger alignment.
